Solving the TTC 2011 Reengineering Case with MOLA and Higher-Order Transformations

The Reengineering Case of the Transformation Tool Contest 2011 deals with automatic extraction of state machine from Java source code. The transformation task involves complex, non-local matching of model elements. This paper contains the solution of the task using model transformation language MOLA. The MOLA solution uses higher-order transformations (HOT-s) to generate a part of the required MOLA program. The described HOT approach allows creating reusable, complex model transformation libraries for generic tasks without modifying an implementation of a model transformation language. Thus model transformation users who are not the developers of the language can achieve the desired functionality more easily.

==> eptcsdata.tex <==
\providecommand{\firstpage}{159}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.15}{10.4204/EPTCS.74.15}}
\pdfoutput=1

